Towards Efficient Convolutional Neural Network for Domain-Specific Applications on FPGA

FPGA becomes a popular technology for implementing Convolutional Neural Network (CNN) in recent years. Most CNN applications on FPGA are domain-specific, e.g., detecting objects from specific categories, in which commonly-used CNN models pre-trained on general datasets may not be efficient enough. This paper presents TuRF, an end-to-end CNN acceleration framework to efficiently deploy domain-specific applications on FPGA by transfer learning that adapts pre-trained models to specific domains, replacing standard convolution layers with efficient convolution blocks, and applying layer fusion to enhance hardware design performance. We evaluate TuRF by deploying a pre-trained VGG-16 model for a domain-specific image recognition task onto a Stratix V FPGA. Results show that designs generated by TuRF achieve better performance than prior methods for the original VGG-16 and ResNet-50 models, while for the optimised VGG-16 model TuRF designs are more accurate and easier to process.

==> tex/motivation.tex <==
\subsection{Motivation and Related Work}

Implementing efficient and effective CNN onto FPGA for domain-specific application is a challenging job,
especially when the major objective is to leverage the benefits of reconfigurable platforms.
Most of the related work focuses on data quantisation and binarisation~\cite{Umuroglu2017, Qiu2016},
arithmetic transformations~\cite{Lu2017}, or
exploiting model sparsity by pruning~\cite{Han2017}.
%Perspectives from recent papers on this topic are mainly about
%data quantisation and binarisation~\cite{Umuroglu2017, Qiu2016},
%exploiting model sparsity by pruning~\cite{Han2017},
%and applying arithmetic transformations~\cite{Lu2017}.
However, 
it is difficult to apply these methods from a domain-specific perspective because
their evaluations and results are based on
specific CNN models and are not guaranteed to be reproducible on other models.
Also, no clear correlation between accuracy
and data representation or sparsity has been discovered yet.
Finally, a sparse CNN model is much harder to process on FPGA
and different sparsity patterns can result in very different performance,
which further limits their employment for domain-specific application.

The motivation of the proposed framework rests on the recent trend
%Our focus in this paper is originated from a recent trend
in efficient CNN architecture design~\cite{Howard2017, Sandler2018, He2015}.
Essentially, the redundancy in CNN is sometimes architectural and can be reduced by replacing
%that the redundancy in CNN is sometime architectural and can be reduced by replacing
the standard convolution layer with efficient convolution \emph{blocks} such as depthwise and pointwise convolution. 
Compared to quantisation and pruning that rely on statistical properties of pre-trained CNN models,
this approach is more generic and has been evaluated
for different domain-specific applications~\cite{Howard2017}.
Unfortunately,
there is no efficient FPGA implementation of these blocks and direct reuse of FPGA designs for standard convolution
cannot exploit their entire potentials.
Therefore, the proposed framework aims at accelerating CNN for domain-specific applications using different architectural approaches
In particular, layer fusion technique is applied during the exploration the design space of a convolution block.
Winograd algorithm is also used to achieve higher performance on spatial convolution.
Finally, data quantisation employed as a complimentary approach to further improving the performance.
%we aim at accelerating CNN for domain-specific applications
%on FPGA through architectural approaches.
%We adapt the layer fusion method to fully explore the design space of
%a convolution block on FPGA platforms,
%and apply Winograd algorithm to achieve higher performance on spatial convolution.
%Data quantisation is complimentary to our approach.

==> tex/related.tex <==
\section{Related Work}\label{sec:related}
